Chain-of-Thought Prompting Elicits Reasoning in Large Language Models

We explore how generating a chain of thought -- a series of intermediate reasoning steps -- significantly improves the ability of large language models to perform complex reasoning. In particular, we show how such reasoning abilities emerge naturally in sufficiently large language models via a simple method called chain of thought prompting, where a few chain of thought demonstrations are provided as exemplars in prompting. Experiments on three large language models show that chain of thought prompting improves performance on a range of arithmetic, commonsense, and symbolic reasoning tasks. The empirical gains can be striking. For instance, prompting a 540B-parameter language model with just eight chain of thought exemplars achieves state of the art accuracy on the GSM8K benchmark of math word problems, surpassing even finetuned GPT-3 with a verifier.

==> fables/commonsense-datasets.tex <==
\begingroup
\begin{table}[t]
    \caption{
    Few-shot exemplars for chain of thought prompting for commonsense reasoning datasets.
    Chains of thought are highlighted.
    Exact prompts with all exemplars are shown in \cref{tab:appendix-commonsenseqa-prompt}--\cref{tab:appendix-sports-understanding-prompt} in the Appendix.
    }
    \small
    \centering
    \begin{tabular}{p{7.8cm}}
        
        \toprule
        \underline{\textbf{\textsc{CommonsenseQA}}} \\
        \vspace{-2mm}
        \textbf{Q:} Sammy wanted to go to where the people were. Where might he go? \\
        Options: \hspace{0.2cm} (a) race track \hspace{0.2cm} (b) populated areas  \hspace{0.2cm} (c) desert\\
        (d) apartment \hspace{0.2cm} (e) roadblock\\
        \vspace{-1mm}
        \textbf{A:} \hl{The answer must be a place with a lot of people. Race tracks, desert, apartments, and roadblocks don't have a lot of people, but populated areas do.} So the answer is (b). \\
        \midrule
        \underline{\textbf{\textsc{StrategyQA}}} \\
        \vspace{-2mm}
        \textbf{Q:} Yes or no: Could a llama birth twice during War in Vietnam (1945-46)? \\
        \vspace{-1mm}
        \textbf{A:} \hl{The War in Vietnam was 6 months. The gestation period for a llama is 11 months. So a llama could not give birth twice during the War in Vietnam.} So the answer is no. \\ 
        \midrule
        \underline{\textbf{\textsc{Date Understanding}}} \\
        \vspace{-2mm}
        \textbf{Q:} The concert was scheduled to be on 06/01/1943, but was delayed by one day to today. What is the date 10 days ago in MM/DD/YYYY? \\
        \vspace{-1mm}
        \textbf{A:} \hl{One day after 06/01/1943 is 06/02/1943, so today is 06/02/1943. 10 days before today is 05/23/1943.} So the answer is 05/23/1943. \\ 
        \midrule
        \underline{\textbf{\textsc{Sports Understanding}}} \\
        \vspace{-2mm}
        \textbf{Q:} Is the following sentence plausible? "Joao Moutinho caught the screen pass in the NFC championship." \\
        \vspace{-1mm}
        \textbf{A:} \hl{Joao Moutinho is a soccer player. The NFC championship is part of American football, not soccer.} So the answer is no. \\
        \bottomrule
    \end{tabular}
    \label{tab:commonsense-datasets}
\end{table}
\endgroup

==> fables/gsm8k-highlight.tex <==
\begin{table}[h]
    \setlength{\tabcolsep}{3.5pt}
    \caption{
    Chain of prompting with \palm{} achieves new state-of-the-art performance on three of five math word problem benchmarks.
    }
    \small
    \centering
    \begin{tabular}{lrrrrr}
        \toprule
          & GSM8K & SVAMP & ASDiv & AQuA & MAWPS \\
         \hline
         Prior best & 55 & 57.4 & 75.3 & 37.8 & 88.4 \\
         \underline{\palm{}} \\
         + Standard prompting & 17.9 & 69.4 & 68.6 & 24.4 & 71.4 \\
         + Chain of thought prompting & \underline{56.9} & \underline{79.0} & 73.9 & 35.8 & \underline{93.3} \\
         \bottomrule
         \\
    \end{tabular}
    \label{tab:gsm8k-highlight}
    \vspace{-3mm}
\end{table}

==> fables/main-gsm8k-examples.tex <==
\definecolor{darkGreen}{rgb}{0.2,0.5,0.2}
\begingroup
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{p{\linewidth}}
        \toprule
        \vspace{-2mm}
        \textbf{\textsc{Question:}} Ducks need to eat 3.5 pounds of insects each week to survive. If there is a flock of ten ducks, how many pounds of insects do they need per day? \\
        \vspace{-1mm}
        \textbf{\textsc{Model Answer \color{darkGreen}{(CORRECT)}:}} Ducks need 3.5 pounds of insects each week. If there is a flock of 10 ducks, then they need 3.5 x 10 = 35 pounds of insects each week. If they need 35 pounds of insects each week, then they need 35 / 7 = 5 pounds of insects each day. The answer is 5. \color{darkGreen}{\checkmark} \\
        \midrule
        \vspace{-2mm}
        \textbf{\textsc{Question:}} It takes Matthew 3 minutes to dig a small hole for shrubs and 10 minutes to dig a large hole for trees. How many hours will it take him to dig 30 small holes and 15 large holes? \\
        \vspace{-1mm}
        \textbf{\textsc{Model Answer \color{darkGreen}{(CORRECT)}:}} It takes Matthew 3 minutes to dig a small hole and 10 minutes to dig a large hole. So it takes Matthew 3 x 30 = 90 minutes to dig 30 small holes. It takes Matthew 10 x 15 = 150 minutes to dig 15 large holes. So it takes Matthew 90 + 150 = 240 minutes to dig 30 small holes and 15 large holes. 240 minutes is 4 hours. The answer is 4 hours. \color{darkGreen}{\checkmark} \\
        \midrule
        \vspace{-2mm}
        \textbf{\textsc{Question:}} I have 10 liters of orange drink that are two-thirds water and I wish to add it to 15 liters of pineapple drink that is three-fifths water. But as I pour it, I spill one liter of the orange drink. How much water is in the remaining 24 liters? \\
        \vspace{-1mm}
        \textbf{\textsc{Model Answer \color{blue}{(INCORRECT)}:}} I have 10 liters of orange drink that are two-thirds water. I have 15 liters of pineapple drink that is three-fifths water. So I have 10 + 15 = 25 liters of drink. I spill one liter of orange drink. So I have 24 liters of drink. 25 - 24 is 1. The answer is 1. \color{blue}{\xmark} \\
        \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{
    Examples of correct and incorrect chains of thought produced by \lamda{} 137B on the GSM8K dataset.
    Even more examples are given in \cref{tab:appendix-gsm8k-correct-examples}--\cref{tab:appendix-gsm8k-incorrect-examples-cont} in the Appendix.
    }
    \label{tab:main-gsm8k-examples}
\end{table}
\endgroup

==> fables/math-ablation.tex <==
\newcommand{\cell}[2]{#1{ \scriptsize $\pm$#2}}
\definecolor{myGreen}{rgb}{0.85,1,0.85}
\definecolor{myRed}{rgb}{1,0.9,0.9}
\newcommand{\rcell}[2]{{#1}{ \scriptsize $\pm$#2}}
\newcommand{\gcell}[2]{{#1}{ \scriptsize $\pm$#2}}

\begin{table}[t]
    \caption{
    Ablation study for different variants of chain of thought, using \lamda{} 137B and \palm{} 540B. 
    }
    \small
    \centering
    \begin{tabular}{lrr}
        \toprule
          & \multicolumn{2}{c}{GSM8K acc. (\%)}  \\
          \cmidrule(lr){2-3}
          & \lamda{} & \palm{} \\
         \hline
         Standard prompting & 6.3 & 17.9 \\
         Chain of thought prompting & 14.8 & 56.5\\
         \underline{Ablations:}   \\
         \hspace{1mm} Equation only & 5.7 & 21.7 \\
         \hspace{1mm} Variable compute only & 6.0 & 17.7 \\
         \hspace{1mm} Thought after answer & 5.9 & 18.0 \\
         \bottomrule
    \end{tabular}
    \label{tab:math-ablation}
    \vspace{-4mm}
\end{table}

==> fables/symbolic-datasets.tex <==
\begingroup
\begin{table}[t]
    \caption{
    Few-shot exemplars for chain of thought prompting for symbolic reasoning datasets.
    Chains of thought are highlighted.
    Exact prompts with all exemplars are shown in \cref{tab:appendix-letter-concat-prompt}--\cref{tab:appendix-coinflip-prompt} in the Appendix.
    }
    \centering
    \small
    \begin{tabular}{p{\linewidth}}
        
        \toprule
        \underline{\textbf{\textsc{Last Letter Concatenation}}} \\
        \vspace{-2mm}
        \textbf{Q:} Take the last letters of the words in "Elon Musk" and concatenate them. \\
        \vspace{-1mm}
        \textbf{A:} \hl{The last letter of ``Elon'' is ``n''. The last letter of ``Musk'' is ``k''. Concatenating them is ``nk''.} So the answer is nk. \\
        \midrule
        \underline{\textbf{\textsc{Reverse List}}} \\
        \vspace{-2mm}
        \textbf{Q:} Reverse the sequence "glasses, pen, alarm, license". \\
        \vspace{-1mm}
        \textbf{A:} \hl{First is glasses. Second is pen. Third is alarm. Fourth is license. Now to reverse, change the order to: Fourth is license. Third is alarm. Second is pen. First is glasses.} So the answer is "license, alarm, pen, glasses". \\ 
        \midrule
        \underline{\textbf{\textsc{Coin Flip}}} \\
        \vspace{-2mm}
        \textbf{Q:} A coin is heads up. Maybelle flips the coin. Shalonda does not flip the coin. Is the coin still heads up? \\
        \vspace{-1mm}
        \textbf{A:} \hl{The coin was flipped by Maybelle. So the coin was flipped 1 time, which is an odd number. The coin started heads up, so after an odd number of flips, it will be tails up.} So the answer is no. \\
        \bottomrule
    \end{tabular}
    \label{tab:symbolic-datasets}
    \vspace{-3mm}
\end{table}
\endgroup
